Honesty is the Best Policy: On the Accuracy of Apple Privacy Labels Compared to Apps' Privacy Policies

Apple introduced privacy labels in Dec. 2020 as a way for developers to report the privacy behaviors of their apps. While Apple does not validate labels, they also require developers to provide a privacy policy, which offers an important comparison point. In this paper, we fine-tuned BERT-based language models to extract privacy policy features for 474,669 apps on the iOS App Store, comparing the output to the privacy labels. We identify discrepancies between the policies and the labels, particularly as they relate to data collected linked to users. We find that 228K apps' privacy policies may indicate data collection linked to users than what is reported in the privacy labels. More alarming, a large number (97%) of the apps with a Data Not Collected privacy label have a privacy policy indicating otherwise. We provide insights into potential sources for discrepancies, including the use of templates and confusion around Apple's definitions and requirements. These results suggest that significant work is still needed to help developers more accurately label their apps. Our system can be incorporated as a first-order check to inform developers when privacy labels are possibly misapplied.

==> additional-data-practices.tex <==
\section{Data Practices Beyond Privacy Labels}
\label{sec:additional-data-practices}

%Apple's privacy labels are designed to inform users about an app's data collection practices. However, 
Privacy policies also cover other privacy-relevant data practices that are not options in the labels. In this section, we highlight a few of these practices and provide insight into additional information that can benefit users but is missing from the privacy labels.

\childrenRatingsCountByPrivacyLabel

\adam{I might argue that we drop this section and move the child apps below into the prior results section. I'm not sure how much this is adding. We do have the space.}

\paragraph{Apps Targeting Children.} 
%Apple does not provide a way for developers to indicate differences in their data collection practices based on app features and audiences. It instead informs users about the potential for such variations in a note below the privacy labels for each app, \textit{``Privacy practices may vary, for example, based on the features you use or your age.''}
%
Developers provide a \textit{Content Rating} as part of the app metadata to indicate the age appropriateness of their apps. These ratings are reviewed by Apple~\cite{Apple:Guidelines}, and used to enforce parental control features that restrict children from accessing the app. 
%
We find that most apps that we analyzed had a 4+ content rating on the App Store (75.98\%; $n=419,762$), while fewer apps had 9+ (0.3\%; $n=16,687$), 12+ (0.8\%; $n=46,737$), or 17+ (1.3\%; $n=69,309$) content rating values. Since privacy labels do not indicate the app's data practices specific to children, the only other option that users have for learning this information is to review the  privacy policy. Given parental control settings, an app with a 4+, 9+, or 12+ rating could be used by minors, although this may not be intended audience for the app. But when an app specifically targets children, it is subject to additional regulation that may require parental consent.
%
%While privacy labels do not specifically describe data practices surrounding children, 
Polisis can identify policy segments that address \textit{International/Specific Audiences} and further identify if the segment addresses \textit{Children}, and then compare this output to the content rating.
%also addresses this audience in their privacy policies.
%
Only 46\% ($n=191,120$) apps with a 4+ content rating also included a privacy policy segment that addresses data practices specific to children. We were more likely to find similar policy segments for apps with different content ratings that can also be accessed by children, 9+ (64\%; $n=10,700$) and 12+ (50\%; $n=23,529$).

We further looked at app content ratings for different privacy label types associated with data collection. These findings are presented in \autoref{fig:children}. Considering apps with a 4+ content ratings, we find that across privacy types, roughly half of these apps had a policy in place that specifically addressed children. While 18\% ($n=75,346$), 37\% ($n=154,972$), and 44\% ($n=184,722$) of the apps with a 4+ content rating declare in their privacy label that they collect data that is used to track users, linked to users, and not linked to user's respectively. Only 53\% ($n=40,081$), 48\% ($n=74,829$), and 49\% ($n=90,755$) of those apps also addressed children in their privacy policies.
%
Adding a 4+ content rating may help developers reach a wider audience, only  half of these apps consider data practices specific to children in the privacy policy. Our findings are a cause for concern, especially in light  of COPPA~\cite{FTC:COPPA:2013} regulations.
%, which is currently going unaddressed due to Apple's lack of regulation.

\dataSecurity
\paragraph{Data Security} While privacy labels provide a way for users to learn  what data is collected by an app and for what purpose, they do not indicate if the data is handled in a secure manner. Polisis can identify segments that address \textit{Data Security}, and further identify if segments that address \textit{Secure data storage} or \textit{Secure data transfer}. 
%
We further considered if apps indicate in their policies that they employ security practices while storing or transferring data and present our findings in \autoref{fig:security}. We find that only 26\% ($n=29,843$) and 33\% ($n=73,051$) of the apps that indicate in their privacy labels that they collect data that is used to track users and linked to users, respectively, also indicate in their privacy labels that they store or transfer data in a secure manner.

\paragraph{Changes to the Privacy Policy.} 
%The App Store does not provide a way for users to be notified of changes to an app's privacy label once the app has been downloaded. 
Apps may choose to notify users of updates to their privacy policies, and we found that 50\% ($n=273,865$) apps that we analyzed addressed the possibility of \textit{privacy-relevant} changes to their policies. However, 38\% ($n=103,070$) of these apps did not indicate a procedure in place to notify users of such changes, and 3\% ($9,173$) explicitly stated that users will receive \textit{no} notification of \textit{privacy-relevant} changes.

For example, the privacy policy from a developer, ChowNow~\cite{ChowNow:Policy}, which has over 3,000 apps in the Apple App Store, places the burden on users, asking that they periodically revisit the policy. The relevant snippet is shown below.

\begin{quote}
    \textit{We may update this Privacy Policy from time to time and without prior notice to you to reflect changes in our privacy practices. We will indicate at the top of this Privacy Policy when it was most recently updated, and we encourage you to revisit this page periodically to stay aware of any changes.}
\end{quote}

\paragraph{Do Not Track Policy.} While 113,921 apps that we analyzed state that they collect data that is used to track users, we identified only 13,183 of these apps that include a \textit{Do Not Track} statement in their privacy policy. Complicating matters, policies may state that they do not honor \textit{Do Not Track} requests from users. An example snippet from \textit{ChowNow}'s policy~\cite{ChowNow:Policy} is provided below.

\begin{quote}
    \textit{As discussed above, third parties such as advertising networks and analytics providers may collect information about your online activities over time and across different websites when you access or use the Services. Currently, various browsers offer a “Do Not Track” option, but there is no standard for commercial websites. At this time, we do not monitor, recognize, or honor any opt-out or do not track mechanisms, including general web browser “Do Not Track” settings and/or signals.}
\end{quote}

\paragraph{User Choice.} Privacy labels do not address choices that users have, leaving them with only the option whether they install the app at all or not. Apps may, however, highlight user choices within their policies. We found that 65\% ($n=360,011$) of the apps that we analyzed addressed user choices over the app's data collection practices. However, 33\% ($n=117,072$) of these apps left users with the only choice of \textit{not} using the service.

==> conclusion.tex <==
\section{Conclusion}

In conclusion, it is rarely a good idea to include the same section three times in a paper, or to have a conclusion that does not conclude.

==> metadata.tex <==
\section{App Store Trends}

In this section, we explore the different properties of apps' metadata and how that intersects with their privacy behavior as reported in their privacy policies and privacy labels. This analysis reveals discrepancies between reported behavior that are specific to certain app types, such as free vs. paid apps, the popularity of the apps (using the number of ratings as a proxy), and the last time the app was updated. Additional analysis was performed based on the content rating, app-size, and release date, but as this analysis did not reveal meaningful results, we provide the comparisons in the appendix. \reminder{add figures to appendix.}


% App costs by privacy type figure.
\appCostsByPrivacyLabel

% App costs.
% Data Used to Track You - Policy Minus Label
% [12.2, -8.0, 13.8, 12.7]
%
% Data Linked to You - Policy Minus Label
% [54.6, 53.4, 80.2, 74.4]
%
% Data Not Linked to You - Policy Minus Label
% [17.0, 5.6, 39.8, 25.8]
%
% Data Not Collected - Policy Minus Label
% [-36.6, -19.7, -73.0, -50.4]
%
\paragraph{App costs.}
%
There are four pricing models on the App Store: free apps, free apps with in-app purchases, paid apps, and paid apps with in-app purchases. 

Interestingly, when only observing privacy labels (the bottom half of \autoref{fig:app-costs-by-privacy}), it would appear that paid apps have better privacy behaviors than their free counter parts. However, the altruism of paid apps compared to free apps disappear when considering  the privacy policies (the top half of \autoref{fig:app-costs-by-privacy}). The privacy policy analysis better aligns with observations of Han et al.~\cite{Han:2019, Han:2020} who compared free and paid apps in the Android Play Store based on inclusion of third-party advertising software, finding no differences between free and paid apps.

As a result of apparent under-reporting by paid apps, we find that this category has the largest discrepancies of potentially under-report data collection practices in their privacy labels, as compared to the privacy policies. The analysis of the privacy policies indicate that 16\% of paid apps collect data used for tracking purposes, whereas only 2\% of those apps report such behavior as part of their  privacy labels. Paid apps also appear to under-report in other categories as well. The privacy policies suggest that 84\% of paid apps collect data linked to users, only 4\% have a privacy label of this type, and when collecting data not linked to users, 55\% have a segment/paragraph in their privacy policy discussing such actions while only 15\% have a privacy label.


% When considering only the developer reported privacy labels it appears that free apps collect, link, and track more data from users, however, when we take into account the privacy policy analysis we find that paid apps have similar data collection behaviors as free apps.
%

%
% Refer to \autoref{fig:app-costs-by-privacy} for full details.



% Ratings counts by privacy type figure.
\ratingsCountByPrivacyLabel

% Rating counts.
% Data Used to Track You - Policy Minus Label
% [9.3, -0.2, -8.8, -16.8, -10.7]
%
% Data Linked to You - Policy Minus Label
% [56.3, 34.7, 33.9, 24.0, 11.4]
%
% Data Not Linked to You - Policy Minus Label
% [16.9, -3.0, -14.0, -15.4, -10.4]
%
% Data Not Collected - Policy Minus Label
% [-36.3, -12.8, -6.1, -2.8, -0.2]
%
\paragraph{Rating counts.}
%
Unfortunately, the App Store meta data does not include download couts, so we use the number of ratings of an app as a proxy for the relative popularity of an app. An app with more ratings likely has more downloads and more users, overall, than an app with fewer ratings. We found that apps with very few ratings (e.g., fewer than 100), were more likely to under-report data collection behaviors on their privacy labels as compared to their privacy policies. For example, according to our privacy policy analysis 29\% of apps with fewer than 100 ($10^2$) user ratings collected data used to track users, while only 19\% of those apps disclosed this in their privacy labels. 
%
We found similar discrepancies in those low-rating count apps when it came to reporting data collected and linked to users: 95\% privacy policy vs. 39\% privacy label, and for data collected but not linked to users, 61\% privacy policy vs. 44\% privacy label. 

The full details can be found in \autoref{fig:ratings-counts-by-privacy}, and the overal trend is that  that less popular apps are more likely to under-reporting their privacy labels as compared to their privacy policy. One possible reason for this discrepancy could be that apps with infrequent ratings and smaller audiences tend to be published by developers with less inclination and incentive for privacy label accuracy. It may also be the case that since Apple has required a privacy policy for longer than privacy labels, the standards for privacy policies are more mature and shared more frequently between less experienced developers. As a result, they contain language that more broadly covers behaviors that the developers are not aware of and do not mark properly in the privacy labels. 
%


% Version date year by privacy type figure.
\versionDateByPrivacyLabel

% Version update date.
% Data Used to Track You - Policy Minus Label
% [8.3, 9.9, 9.3, 12.2, 17.8, 5.1]
%
% Data Linked to You - Policy Minus Label
% [52.3, 60.1, 66.3, 61.8, 45.0, 49.9]
%
% Data Not Linked to You - Policy Minus Label
% [13.3, 20.1, 21.3, 24.2, 39.0, 40.9]
%
% Data Not Collected - Policy Minus Label
% [-32.0, -40.0, -48.2, -46.7, -27.3, -33.5]
%
\paragraph{Version update date.}
After Decembner 2020, all new apps and app updates to the App store require the developr to include a privacy label. 
%
Pre-existing apps can also add and update their privacy labels without updating the app (i.e., without increasing the version number) by submitting a revision to their App Store page. Essentially, these are developers simply choosing to come into compliance with the new policy without being forced to due to a version update to their app.  We can then consider the date  of the last version update as a proxy for how and when a developer came into compliance with the policy: an app with a version update after December of 2020 with privacy labels added it by choice, not because they were required to do so. 

In \autoref{fig:version-date-by-privacy} we report the findings of privacy labels and policies organized by the year of the last version update. There is large discrepancies across the board between the privacy labels and policies, but interestingly, in some categories, older version-updated apps (<2018) show less discrepancies when considering data collected that is linked or used to track users compared to apps more recently updated. However, older version-updated apps tend to be less accurate when reporting data not linked to users, perhaps due to great confusion regarding data collection practices with respect app analytics and unique identifiers with privacy labels by choice, as discussed previously, and thus may have made a better effort to accurate reflect correct behavior. The differences for data not linked is likely caused by the same confusion over privacy labels categories regarding analytic or other purpose of data collection with unique identifiers. \adam{We should consider dropping this section ... not sure if the through line is clear}


%, apps whose last update occurred prior to, and including, 2019, a and those choose to add privacy labels, , show 42\% track user data, but only 37\% of those apps reported this in their privacy label. 
% 
%A similar difference is found with linked data, 94\% privacy policy versus 44\% privacy label, and unlinked data with 66\% in the privacy policy and 26\% in the labels.  \adam{I don't buy this, all the update dates are off everywhere?!?}
%
%This result suggests that apps with limited developer support with regards to software updates are less likely to keep up with their privacy label accuracy.
%
%You may find the full results in \autoref{fig:version-date-by-privacy}. 

%\appSizeByPrivacyLabel
%\contentRatingByPrivacyLabel
%\releaseDateByPrivacyLabel
%\appStoreGenreTopFiveByPrivacyType
%\appStoreGenreByPrivacyType
